Cross-Lingual Transfer of Semantic Roles: From Raw Text to Semantic Roles

We describe a transfer method based on annotation projection to develop a dependency-based semantic role labeling system for languages for which no supervised linguistic information other than parallel data is available. Unlike previous work that presumes the availability of supervised features such as lemmas, part-of-speech tags, and dependency parse trees, we only make use of word and character features. Our deep model considers using character-based representations as well as unsupervised stem embeddings to alleviate the need for supervised features. Our experiments outperform a state-of-the-art method that uses supervised lexico-syntactic features on 6 out of 7 languages in the Universal Proposition Bank.

==> analysis_tables.tex <==
\newcolumntype{d}[1]{D..{#1}}
\newcommand\mc[1]{\multicolumn{1}{c}{#1}} %

\begin{table*}
\begin{subtable}[t]{0.48\textwidth}
\scriptsize
\centering

\setlength{\tabcolsep}{5pt}
\begin{tabular} {l | c c c c c }
\hline \hline
Pred. Arg. & Char & Stem & Lemma & Sup. & Freq. \\ \hline
 Nominal A0 & 62.4 & 51.9 & 58.6 & 69.2 & 1.8 \\ 
 Nominal A1 & 48.4 & 41.3 & 45.8 & 52.5 & 1.9 \\ 
 Nominal A2 & 6.5 & 5.9 & 6.5 & 51.3 & 1.9 \\ 
 Nominal AM* & 30.7 & 32.3 & 31.1 & 48.7 & 2.6 \\ 
 Verbal A0 & 64.5 & 61.2 & 61.1 & 76.0 & 20.6 \\ 
 Verbal A1 & 56.5 & 57.3 & 55.9 & 70.9 & 30.2 \\ 
 Verbal A2 & 38.7 & 39.0 & 38.2 & 58.8 & 11.7 \\ 
 Verbal AM* & 28.1 & 29.0 & 29.9 & 53.1 & 28.5 \\
 \hline \hline
 \end{tabular}
 \caption{\footnotesize German}
\label{tab:table1_a}
\end{subtable}
\hspace{\fill}
\begin{subtable}[t]{0.48\textwidth}
\flushright
\scriptsize
\centering

\setlength{\tabcolsep}{5pt}
\begin{tabular} {l | c c c c c }
\hline \hline
Pred. Arg. & Char & Stem & Lemma & Sup. & Freq. \\ \hline
 Nominal A0 & 44.4 & 25.0 & 44.4 & 52.6 & 0.7 \\ 
 Nominal A1 & 50.8 & 54.5 & 54.0 & 55.8 & 1.3 \\ 
 Nominal A2 & 28.6 & 28.6 & 33.3 & 60.0 & 1.3 \\ 
 Nominal AM* & 35.9 & 21.6 & 22.2 & 50.0 & 1.2 \\ 
 Verbal A0 & 43.7 & 45.6 & 42.7 & 64.3 & 14.6 \\ 
 Verbal A1 & 62.3 & 61.7 & 60.3 & 73.0 & 36.7 \\ 
 Verbal A2 & 37.1 & 38.8 & 38.9 & 61.5 & 12.4 \\ 
 Verbal AM* & 27.9 & 28.4 & 28.6 & 54.9 & 31.4 \\ 
 \hline \hline
  \end{tabular}
\caption{\footnotesize Spanish}
\label{tab:table1_b}
\end{subtable}

\bigskip 

\begin{subtable}[t]{0.48\textwidth}
\scriptsize
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular} {l | c c c c c }
\hline \hline
Pred. Arg. & Char & Stem & Lemma & Sup. & Freq. \\ \hline
Nominal A0 & 36.4 & 45.5 & 43.5 & 71.4 & 0.5 \\ 
Nominal A1 & 41.4 & 46.7 & 45.6 & 45.2 & 1.0 \\ 
Nominal A2 & 0.0 & 0.0 & 0.0 & 15.4 & 1.0 \\ 
Nominal AM* & 30.3 & 26.7 & 20.7 & 30.8 & 0.7 \\ 
Verbal A0 & 56.0 & 54.0 & 54.3 & 73.6 & 12.3 \\ 
Verbal A1 & 58.7 & 57.2 & 58.4 & 68.8 & 34.3 \\ 
Verbal A2 & 37.3 & 35.7 & 39.0 & 57.8 & 17.3 \\ 
Verbal AM* & 27.8 & 29.9 & 27.6 & 50.3 & 31.0 \\
 \hline \hline
 \end{tabular}
 \caption{\footnotesize Finnish}
\label{tab:table1_c}
\end{subtable}
\hspace{\fill}
\begin{subtable}[t]{0.48\textwidth}
\flushright
\scriptsize
\centering

\setlength{\tabcolsep}{5pt}
\begin{tabular} {l | c c c c c }
\hline \hline
Pred. Arg. & Char & Stem & Lemma & Sup. & Freq. \\ \hline
Nominal A0 & 83.3 & 71.4 & 83.3 & 83.3 & 0.6 \\ 
Nominal A1 & 66.7 & 66.7 & 66.7 & 66.7 & 1.1 \\ 
Nominal A2 & 0.0 & 0.0 & 0.0 & 0.0 & 1.1 \\ 
Nominal AM* & 40.0 & 50.0 & 57.1 & 40.0 & 0.3 \\ 
Verbal A0 & 59.8 & 59.7 & 60.8 & 87.3 & 32.4 \\ 
Verbal A1 & 58.9 & 58.0 & 58.7 & 81.4 & 48.3 \\ 
Verbal A2 & 37.9 & 39.3 & 38.1 & 67.9 & 8.0 \\ 
Verbal AM* & 5.9 & 5.5 & 5.2 & 53.3 & 8.9 \\
 \hline \hline
 \end{tabular}
 \caption{\footnotesize French}
\label{tab:table1_d}
\end{subtable}

\bigskip 

\begin{subtable}[t]{0.48\textwidth}
\scriptsize
\centering

\setlength{\tabcolsep}{5pt}
\begin{tabular} {l | c c c c c }
\hline \hline
Pred. Arg. & Char & Stem & Lemma & Sup. & Freq. \\ \hline
Nominal A0 & 25.0 & 44.4 & 33.3 & 73.7 & 0.5 \\ 
Nominal A1 & 63.2 & 63.2 & 55.0 & 54.1 & 0.8 \\ 
Nominal A2 & 0.0 & 0.0 & 0.0 & 25.0 & 0.8 \\ 
Nominal AM* & 25.0 & 34.5 & 28.6 & 46.7 & 0.7 \\ 
Verbal A0 & 38.8 & 37.9 & 39.3 & 66.7 & 14.1 \\ 
Verbal A1 & 65.4 & 64.3 & 65.4 & 77.0 & 35.2 \\ 
Verbal A2 & 31.9 & 31.7 & 33.3 & 59.8 & 14.2 \\ 
Verbal AM* & 25.1 & 25.9 & 25.6 & 58.0 & 30.2 \\
 \hline \hline
 \end{tabular}
 \caption{\footnotesize Italian}
\label{tab:table1_e}
\end{subtable}
\hspace{\fill}
\begin{subtable}[t]{0.48\textwidth}
\flushright
\scriptsize
\centering

\setlength{\tabcolsep}{5pt}
\begin{tabular} {l | c c c c c }
\hline \hline
Pred. Arg. & Char & Stem & Lemma & Sup. & Freq. \\ \hline
Nominal A0 & 35.0 & 29.2 & 37.6 & 34.5 & 1.2 \\ 
Nominal A1 & 30.9 & 33.2 & 33.0 & 32.3 & 1.8 \\ 
Nominal A2 & 11.1 & 10.3 & 13.8 & 28.6 & 1.8 \\ 
Nominal AM* & 18.7 & 19.4 & 18.5 & 22.2 & 2.2 \\ 
Verbal A0 & 48.1 & 49.0 & 48.6 & 50.7 & 17.9 \\ 
Verbal A1 & 63.4 & 63.0 & 63.3 & 53.4 & 34.0 \\ 
Verbal A2 & 41.2 & 42.7 & 41.1 & 43.6 & 10.9 \\ 
Verbal AM* & 26.3 & 27.8 & 27.3 & 28.2 & 29.5 \\
 \hline \hline
 \end{tabular}
 \caption{\footnotesize Portuguese}
\label{tab:table1_f}
\end{subtable}

\bigskip 

\begin{subtable}[t]{0.48\textwidth}
\scriptsize\centering

\setlength{\tabcolsep}{5pt}
\begin{tabular} {l | c c c c c }
\hline \hline
Pred. Arg. & Char & Stem & Lemma & Sup. & Freq. \\ \hline
Nominal A0 & 20.5 & 16.7 & 11.8 & 44.4 & 1.2 \\ 
 Nominal A1 & 8.1 & 8.2 & 5.8 & 42.9 & 2.1 \\ 
 Nominal A2 & 0.0 & 0.0 & 0.0 & 50.0 & 2.1 \\ 
 Nominal AM* & 12.9 & 0.0 & 0.0 & 37.5 & 0.8 \\ 
 Verbal A0 & 21.5 & 19.3 & 20.9 & 52.5 & 23.0 \\ 
 Verbal A1 & 25.9 & 24.9 & 19.9 & 52.5 & 38.3 \\ 
 Verbal A2 & 14.7 & 11.9 & 12.4 & 40.5 & 13.7 \\ 
 Verbal AM* & 10.2 & 9.6 & 11.3 & 30.4 & 18.3 \\
 \hline \hline
 \end{tabular}
 \caption{\footnotesize Chinese}
\label{tab:table1_g}
\end{subtable}
\hspace{\fill}
% \begin{subtable}[t]{0.48\textwidth}
% \flushright
% \scriptsize
% \setlength{\tabcolsep}{5pt}
% \begin{tabular} {l | c c c c c }
% \hline \hline
% System & Char & Stem & Lemma & Sup. & Freq. \\ \hline
% Nominal A0 & 35.0 & 29.2 & 37.6 & 34.5 & 1.2 \\ 
% Nominal A1 & 30.9 & 33.2 & 33.0 & 32.3 & 1.8 \\ 
% Nominal A2 & 11.1 & 10.3 & 13.8 & 28.6 & 1.8 \\ 
% Nominal AM* & 18.7 & 19.4 & 18.5 & 22.2 & 2.2 \\ 
% Verbal A0 & 48.1 & 49.0 & 48.6 & 50.7 & 17.9 \\ 
% Verbal A1 & 63.4 & 63.0 & 63.3 & 53.4 & 34.0 \\ 
% Verbal A2 & 41.2 & 42.7 & 41.1 & 43.6 & 10.9 \\ 
% Verbal AM* & 26.3 & 27.8 & 27.3 & 28.2 & 29.5 \\
%  \hline \hline
%  \end{tabular}
%  \caption{\footnotesize Portuguese}
% \label{tab:table1_f}
% \end{subtable}


\caption{Performance of different systems (unsupervised lemma with char BiLSTM (``char''), unsupervised stemmer (``stem''), supervised lemmas (``lemma''), and the supervised results (``sup.'')) for different semantic roles. Results are shown for nominal and verbal predicates separately.}
\label{tab:analysis_results}
\end{table*}

==> confusion_matrix.tex <==
\begin{table}
\small
\begin{tabular}{l| c c c c c c }
\hline
   & {\bf A0} & {\bf A1} & {\bf A2} & {\bf A3} & {\bf AM} & \tt{NULL} \\
\hline
\hline
{\bf A0} &   0.7 &   0.1  &     0.0 &   0.0 &   0.0 &   0.2 \\
{\bf A1} &   0.0 &   0.7 &   0.0 &   0.0 &   0.0 &  0.3 \\   
{\bf A2} &   0.0 &   0.1 &   0.7 &   0.0 &   0.0 &   0.1 \\
{\bf A3} &   0.0 &   0.0 &   0.0 &   1.0 &   0.0 &  0.0 \\
{\bf AM} &   0.0 &   0.0 &   0.1 &   0.0 &   0.6 &   0.3 \\   
\tt{NULL}: &   0.0 &   0.0 &   0.0 &   0.0 &   0.0 &  1.0 \\
\hline
\end{tabular}
\caption{Confusion matrix of our system for French}\label{table:confusion_matrix}
\end{table}

==> table_conll.tex <==
\begin{table*}[]
\centering
\label{table:conll}
%\small
\setlength{\tabcolsep}{5pt}

\begin{tabular}{ll ccccc c c c c c c }
\hline
\hline

\multirow{2}{*}{System} &  & \multicolumn{5}{c}{Features} & & \multicolumn{5}{c}{Languages}\\
&  & {\scriptsize POS} & {\scriptsize Lemma} & {\scriptsize Syntax} & {\scriptsize Sense} & {\scriptsize Global} &  & en & de & es & cs & zh \\
 \cline{1-1} \cline{3-7} \cline{9-13}
\newcite{bj_sup} &  & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} &  &  86.9 & 79.7 & 76.5 & 85.4 & 78.6\\ 
\newcite{lei-EtAl:2015:NAACL-HLT}   &  & \ding{51}  & &\ding{51} &  & &  &  86.6 & -- & -- & -- & --   \\
\newcite{fitzgerald-EtAl:2015:EMNLP}&  &  \ding{51}  &   & \ding{51}  &   & \ding{51} &  &  87.3 & -- & -- & -- & --    \\
\newcite{roth_sup} &   &  \ding{51} &  &   \ding{51} &   &  \ding{51} &  &  87.7 & 80.1 & 80.2 & -- & 79.4 \\ 
\newcite{marcheggiani-2017} &  &  \ding{51} & \ding{51} &  &  & &  &  87.7 & -- & 80.3 & 86.0 & 81.2 \\
\newcite{marcheggiani-titov:2017:EMNLP2017} & & \ding{51} & \ding{51} & \ding{51} & & & &  88.0 & -- & -- & -- & 82.5 \\
\newcite{marcheggiani-titov:2017:EMNLP2017} & & \ding{51} & \ding{51} & \ding{51} & &\ding{51}  & &  89.1 & -- & -- & -- & -- \\
\cline{1-1} \cline{3-7} \cline{9-13}
Ours (supervised lemma) &  &  & \ding{51} & & & &   &  \textbf{89.3} & 76.7 & \textbf{ 82.0} & \textbf{86.3} & 82.7 \\
Ours (character BiLSTM)  &  &  & & & & &   & 88.5 & 74.9 & 78.9 & 86.0 & \textbf{82.9} \\

\hline
\hline

\end{tabular}
\caption{Results on CoNLL 2009 in-domain test set compared to other supervised systems. All results show labeled F-score obtained using standard CoNLL 2009 evaluation script. Our predicted senses come from the best predictions in the CoNLL shared task~\protect\cite{conll2009_shared}. Columns in the middle indicate if POS, lemma, Syntax and Sense are used as the feature to build the model. }\label{table:sup:results}
\end{table*}

==> table_param.tex <==
\begin{table}[t!]
\centering
\label{table:param}
%\small
%\setlength{\tabcolsep}{2pt}
\begin{tabular}{ll}
\hline\hline
Hyperparameter & Size \\
\hline
Word embedding ($d_w$) & 100 \\
Character embedding ($d_c$) & 50  \\
LSTM hidden state ($d_h$) & 512 \\
Input lemma vector ($d_{le}) $ & 100 \\
Role embedding ($d_r$) & 128 \\
Decoder lemma vector ($d'_l$) & 128\\
Char LSTM hidden state ($d_{ch}$) & 100\\
Minibatch size & $\sim$1K tokens \\
Learning rate (Adam) & $0.001$ \\
\hline\hline

\end{tabular}
\caption{Parameters in our SRL model.}\label{table:paremeters}
\end{table}

==> table_proj_2.tex <==
\begin{table*}[t!]
\centering
\label{table:proj}
%\small
 %\setlength{\tabcolsep}{3pt}
 
\begin{tabular}{l c c c cccc}
\hline\hline

System & de &  es & fi & fr & it & pt & zh\\
\hline

ARD &
59.8 \scriptsize{(55.0)} & 60.6 \scriptsize{(52.2)} & 59.0 \scriptsize{(53.1)} & 71.0 \scriptsize{(63.4)} &  59.2 \scriptsize{(52.3)} & 61.2 \scriptsize{(53.9)} & 50.3 \scriptsize{(42.5)}\\
Sup. lemma & 61.7 \scriptsize{(57.0)} & 62.4 \scriptsize{(55.7)} & 62.5 \scriptsize{(59.2)} & 65.0 \scriptsize{(58.9)} & 61.8 \scriptsize{(56.4)} & 63.0 \scriptsize{(56.8)}  & 52.1 \scriptsize{(43.7)}\\
Unsup. stem & 62.0 \scriptsize{(57.4)} & 63.0 \scriptsize{(56.0)} & 64.5 \scriptsize{(58.8)} & 65.3 \scriptsize{(59.2)} & 61.3 \scriptsize{(55.4)} & 62.8 \scriptsize{(56.8)} & 52.6 \scriptsize{(43.2)}\\

\hline
{\bf Our Model} & 61.0 \scriptsize{(57.0)} & 62.5 \scriptsize{(56.0)} & 64.6 \scriptsize{(58.9)} & 65.1 \scriptsize{(58.5)} & 61.0 \scriptsize{(55.5)} & 62.9 \scriptsize{(56.5)} & 52.7 \scriptsize{(42.7)}\\
\hline
Supervised & 74.5 \scriptsize{(72.0)} & 77.8 \scriptsize{(75.2)} & 74.0 \scriptsize{(69.6)} & 88.9 \scriptsize{(87.5)} &77.9 \scriptsize{(75.9)}& 66.6 \scriptsize{(62.4)} & 68.8 \scriptsize{(68.6)} \\

\hline\hline

\end{tabular}

\caption{Results of the projection experiments on the Universal PropBank test sets compared to different baselines: the second column shows results of the bootstrapping SRL system proposed in \cite{aminian-rasooli-diab:2017:I17-2}, the third and second columns shows results of the systems with supervised and unsupervised lemmas respectively. Numbers in parenthesis show results with automatic predicate senses.}\label{table:proj:results}   

\end{table*}

==> table_super.tex <==
\begin{table*}[]
\centering
\label{table:super}
\small
\begin{tabular}{llllllllllllllll}
   &\multicolumn{2}{c}{$lem^{+}pos^{+}$}&&\multicolumn{2}{c}{$lem^{-}pos^{+}$}&&\multicolumn{2}{c}{$lem^{-}pos^{+}$}&&\multicolumn{2}{c}{$lem^{-}pos^{-}$} & &\multicolumn{2}{c}{$lem^{-}$}\\
   \hline 
    \hline
    & goldPS & autoPS & & goldPS & autoPS &  & goldPS & autoPS & &  goldPS & autoPS &  & goldPS & autoPS\\
    \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} \cline{14-15}
de &74.51 & 72.06 & & 73& 70.94 & & 74.58 & 73.12 & & 73.23 & 71.25 & & 73.54 & 71.59 &\\

es & 77.78 & 75.19  & & 77.03 & 73.76 & & 76.89 & 74.34 & & 75.27 & 72.32 & & 75.43 & 72.48 \\

fi & 74.08 & 69.59 & & 70.68 & 67.59 & & 73.68 & 72.42 & & 72.39 & 69.94 & & 70.2 & 67.7\\

fr & 88.87 & 87.53 & & 87.08 & 85.69 & & 88.21 & 86.54 & & 87.95 &  85.74 & & 87.47 & 85.24 \\

it & 77.88 & 75.95 & & 77.19 &  74.54 & & 77.3 & 75.42 & & 74.13 &  71.77 & & 75.02 & 72.68\\

pt & 66.58 & 62.45 & & 66.57 & 58.28 & & 62.94 &  59.67 & & 64.86  & 58.65 &  &63.21 & 56.54 \\

zh & 68.77 & 68.6 & & 67.24 & 66.93 & & 65.68 & 65.39 & & 65.74 & 65.45 & & 64.26 & 63.97  \\  
\hline
\end{tabular}
\caption{Results of supervised experiments on Universal PropBank for different setups. GoldPS shows results when we use gold predicate sense for evaluation and autoPS shows results when automatic predicate sense is used for evaluation.}
\end{table*}

==> table_uni_test_stats.tex <==
\begin{table*}[t!]
\centering
%\small
%\setlength{\tabcolsep}{2pt}
\begin{tabular}{llllllll}
Language & de & es & fi & fr & it & pt & zh \\
\hline\hline
\#Sentences & 977 & 274 & 648 & 298 & 489 & 936 & 500 \\
\#Tokens & 16K & 8K & 9K  & 7K & 11K  & 22K  & 12K \\
\#Types & 5K & 3K & 4K & 2K & 3K & 6K & 4K \\
\#Predicates & 1K & 847 & 1K & 635 & 1K  & 2K & 1K \\
\hline
\end{tabular}
\caption{Sizes of treebanks in the Universal Propbank test data for all languages.}\label{table:uni_test_stats}
\end{table*}
